Learning Planning-based Reasoning by Trajectories Collection and Process Reward Synthesizing

Large Language Models (LLMs) have demonstrated significant potential in handling complex reasoning tasks through step-by-step rationale generation. However, recent studies have raised concerns regarding the hallucination and flaws in their reasoning process. Substantial efforts are being made to improve the reliability and faithfulness of the generated rationales. Some approaches model reasoning as planning, while others focus on annotating for process supervision. Nevertheless, the planning-based search process often results in high latency due to the frequent assessment of intermediate reasoning states and the extensive exploration space. Additionally, supervising the reasoning process with human annotation is costly and challenging to scale for LLM training. To address these issues, in this paper, we propose a framework to learn planning-based reasoning through Direct Preference Optimization (DPO) on collected trajectories, which are ranked according to synthesized process rewards. Our results on challenging logical reasoning benchmarks demonstrate the effectiveness of our learning framework, showing that our 7B model can surpass the strong counterparts like GPT-3.5-Turbo.

==> latex/impact.tex <==
\section*{Impact Statements}
This paper explores a approach to synthesize process rewards, which is employed to improve the reliability and faithfulness of reasoning process via direct preference optimization. We plan to release the model weights and trajectory data distilled from GPT-4/GPT-3.5-Turbo. However, since our experiments are conducted under task-specific training, there should be no direct potential societal consequences. There are many potential indirect societal consequences of our work, none of which we feel must be specifically highlighted here.


==> latex/intro_icml.tex <==
\section{Introduction}
\label{sec:intro}
\input{images/example}

% \ZY{Why reasoning capability is important?} 
Natural language reasoning has been a fundamental element in the advancement of artificial intelligence (AI), with its significant impact on a variety of applications including planning and decision making~\citep{reasoning-llm-survey}. The goal of building AI systems capable of replicating human-like reasoning remains a primary focus within the research community.
% \fk{Reasoning has long been recognized as an important ability representing human intelligence, and it plays an essential roles in various applications, like planning and decision making~\citep{reasoning-llm-survey}.
% Recent advancements of Large Language Models (LLMs) have demonstrated their potential in solving complex tasks by generating reasoning step chains.}
% However, LLMs are proven to easily generate falsehood rationales~\citep{gpt4-sparks,cot-faithful-anthrophic}, which further lead to incorrect results under the complex reasoning scenarios~\citep{alert,reasoning-llm-survey,logic-llm}.
% Natural language reasoning has long been a critical aspect in building artificial intelligence, which plays a pivotal role in numerous applications, including planning and decision-making~\citep{reasoning-llm-survey}.
% building system capable of reasoning has always been the long-term goal of research community, as highlighted in various studies.
% \ZY{add a transition from human reasoning to machine reasoning.} 
% The recent progress in Large Language Models (LLMs) has showcased their capability to tackle intricate tasks by formulating reasoning step chains. Despite these advances, it has been established that LLMs can inadvertently produce misleading rationales~\citep{gpt4-sparks,cot-faithful-anthrophic}, leading to inaccurate outcomes, particularly in complex reasoning scenarios~\citep{alert,reasoning-llm-survey,logic-llm}.
Recent advancements in Large Language Models (LLMs) have showcased their ability to perform complex reasoning tasks, creating sequences of reasoning steps akin to human thought processes~\citep{cot,least-to-most}. Despite these advancements, it is also  concerning that LLMs are susceptible to generating misleading rationales \citep{gpt4-sparks,cot-faithful-anthrophic}. Such inaccuracies are particularly pronounced in complex reasoning scenarios \citep{alert,reasoning-llm-survey,logic-llm}, underscoring a significant challenge.
% refining these models to better mirror the nuanced, context-sensitive reasoning abilities inherent in humans.
% Large language models (LLMs) have shown their capability in solving complex reasoning tasks by generating solutions in a chain-of-thought format~\citep{cot}.

Tremendous efforts have been dedicated to improve the reliability and faithfulness of generated rationales. One way is to incorporate \emph{process supervision}. For example, ~\citet{wizardllm}, \citet{wizardmath} and \citet{mammoth} propose to sample diverse rationales from a larger teacher LLM to perform distillation \citep{kd2015hinton} of knowledge  about reasoning, and \citet{shinn2023reflexion} employ LLMs themselves for self-correction to each intermediate reasoning step.
% Tremendous efforts have been dedicated to improving the reliability and faithfulness of generating rationales. One way to achieve this is to incorporate process supervision from either stronger LLMs or human experts.
% including fine-tuning on the sampled rationales from larger models~\citep{wizardllm,wizardmath,mammoth} and self-correction~\citep{shinn2023reflexion}. 
% However, these methods always seek help from GPT-4 or other stronger LLMs as the teacher model to discover potential flaws or annotate better reasoning processes, \fk{which has inhibited the possibility for continuous improvements.}
Yet, these approaches predominantly rely on LLMs for identifying errors or providing superior reasoning processes, which could be limited by their capacity. %, this reliance may hinder the potential for ongoing advancements.
% \ZY{Why these methods are not good enough?}
% Another important direction lies in incorporating process supervision~\citep{prm-and-orm}. \citet{lets-verify} trains a process-supervised reward model (PRM) using the step-level feedback over model-generated solutions, which is annotated by human experts. The policy model can thus be optimized through the feedback of the PRM.
% Process-supervision is verified to yield better results, which, however, often leads to more expensive cost than simply annotating final outcome.
An alternative is to consider \emph{human} process supervision~\citep{prm-and-orm}. For instance, \citet{lets-verify} propose to train a process-supervised reward model (PRM) using step-level feedback on model-generated solutions, which is annotated by human experts. This enables LLMs to refine their rationales based on the PRM's feedback. While human process supervision has proven effective, it often incurs higher costs compared to mere final outcome annotation as well as the automatic process annotation from a teacher LLM.
% And it is usually much easier to simply judge the correctness of the final answer rather than writing or evaluating a complete trajectory for human experts.
% One leading direction is to introduce external search to avoid local minimum of auto-regressive decoding, which typically requires a critic model estimating the expected value of each state to find a better solution~\citep{tree-of-thought}.
% either by searching a better way to prompt LLMs~\citep{react,shinn2023reflexion,rap}, or introducing self-verification/feedback~\citep{xie2023self-eval-decoding} as extra constraints to export better rationales.

% \ZY{Despite what? and here the `another direction` is a bit confusing.}
% Despite the fully data-driven approaches, another direction is transforming reasoning into planning problem, and augmenting the auto-regressive decoding process with value-based search~\citep{tree-of-thought}.
% \fk{Addressing the limitations of rationale annotation and the opaque reasoning process of LLMs, some research efforts are exploring alternatives to the auto-regressive paradigm. One such approach models the reasoning process akin to planning, wherein an optimal reasoning path is constructed through reward-based search~\citep{tree-of-thought}.}
In addition to the attempts on process supervision, some research efforts have explored approaches to mitigate the weakness of greedy decoding that the reasoning process can hardly be adjusted when it reaches an unexpected state. In other words, the model should be able to forecast the future states and consider the optimal reasoning path in a boarder exploration space.
% Recently, some work tries to align the reasoning process with planning~\citep{rap,react}, which can explicitly introduce the problem decomposition process. Like the behaviour of intelligent agent, planning based reasoning can not only reduce the difficulty by decomposing the problem into smaller ones, but also provide format and clear rationales.
% \citet{rap} have introduced a basic framework of reasoning-as-planning (RAP), where the rationale is defined as the Markov Decision Process. Each step can either be the current state, e.g., all intermediate results in arithmetic reasoning, and all known facts in hypothesis verification, or the action to be taken, such as selecting another group of arguments for calculation (arithmetic reasoning), or introducing a new rule to derive new facts (hypothesis verification).
\citet{rap} introduce a general framework of reasoning-as-planning (RAP), where the reasoning process is defined as a Markov Decision Process (MDP). 
% Each step in the MDP can either be the current reasoning state, or the next action to be taken 
{Each step in the MDP comprises a \textit{state}-\textit{action} pair, whose particular implementation can vary with different application scenarios.}
% \sj{this sentence needs more clarity (better to revise it based on the standard MDP definition.}
For example, in arithmetic reasoning, an MDP step includes a state that summarizes all the known variables and an action can be  calculating the value of an unknown variable.
% Figure~\ref{fig:example} shows the process of logical reasoning, where the reasoning states can be known facts and rules, and the action is the next group of facts and rules to derive a new conclusion.
% During inference, each state-action group will receive a reward provided by another LLM, or external verifier. The planning process is conducted under the guidance of Mento Carlo Tree Search (MCTS), which maximizes the rewards received along the trajectory while compressing the search space.
Figure~\ref{fig:example}  illustrates this process in the context of logical reasoning using the ReAct~\citep{react} format. At each step the agent can  \emph{Think} (optionally) and \emph{Act}, which involves selecting a group of facts and rules to deduce a new conclusion.\footnote{The notion of \emph{action} subsumes both thinking and acting.} It can optionally make an \textit{Observation} to get an ``updated view'' of the state. %\footnote{\fk{Sometimes the \textit{Thought} and \textit{Observation} can be absent.  In this case, the absent statement is often integrated into the last one, e.g., \textit{Action 1} entails \textit{Observation 1} in Figure~\ref{fig:example}. Although it is not as strict as the original ReAct, we still keep these samples to obtain larger dataset.}}
%is treated as \textit{state} constituted by known facts and rules.}
% Known facts and rules constitute the reasoning states, and the action involves selecting a group of these facts and rules to deduce a new conclusion.
During inference, each state-action pair is assigned a reward, either by an LLM or  external verifier. The planning process is steered by a Monte Carlo Tree Search (MCTS) \citep{mcts}, which aims to maximize the {expected total cumulative} reward (or utility) obtained along the chosen path while effectively narrowing the search space {(Figure~\ref{fig:micro-frame}(a))}.

% Yet, as discussed previously, the approaches are approaching to the internal upper bound, instead of really advancing it. Some investigations also prove that self-evaluation/feedback can be really unreliable when being applied to complex reasoning tasks~\citep{cant-self-correct}.
% Existing RAP frameworks often ignore the real feedback, i.e., the limited critique come from LLMs themselves, which can lead to biased and unreliable estimation of rewards.
Existing RAP frameworks often assume LLMs as the world model being able to assess the quality of each reasoning step.
As a result, the online planning may introduce huge latency and cost due to frequent assessments of intermediate states and the large search space.
% As a consequence, though promising, it is more basic and essential to answer how well can LLMs learn from limited and sparse expert feedback, and is it possible to approximate the process reward via merely outcome supervision.
% Besides, the estimation of expected value for each node in MCTS relies on frequent attempts, leading to heavy latency brought by generating and evaluating different trajectories.
% \ZY{Not link well with the writing logic of abstract.}
% To this end, one natural question is that is it possible to imitate the process supervision process in RAP, and combine it with the data-driven approach to bypass the inference cost.
Nevertheless, we find that the core idea behind planning-based reasoning is to employ online simulation by taking few forward steps to find the optimal path, {and the evaluation becomes more accurate when it has access to real outcome feedback.}
% which plays a similar role with process supervision. 
% \sj{how is it similar? Not clear.}
% In order to address the problems mentioned above, in this paper, we propose to combine the advantages from process-supervision and reasoning-as-planning.
% In order to answer this question, 
%Motivated from this, 
% in this paper, we have explored synthesized reward supervision by collecting offline positive and negative trajectories to develop a reward model for reinforcement learning.


In this paper, we explore \emph{offline simulation} to synthesize process supervision. We introduce ground-truth outcome supervision that we back-propagate to intermediate states instead of relying on LLMs  for process assessment.
% \ZY{Is it possible to add a simple scheme for illustration?}
% Besides, the back-propagation operation in MCTS to update the expected value of each state is calibrated by introducing the ground-truth outcome supervision. 
We develop a simple and effective strategy based on partial trajectory exploration.
We first collect some solutions from LLMs as the seed trajectories, and then sample several intermediate reasoning states from them as the non-leaf nodes in planning. After that, the LLMs are asked to retry to complete each of them multiple times by taking the intermediate states as new starting points of reasoning.
We take the number of completions that have reached the correct outcome as the estimate of expected utility. %\sj{Following this, we can train a process-supervised reward model based on the collected coarse signals to reduce both the noise and annotation cost by exploration.} \sj{$\rightarrow$ why do you need to train a PRM? The whole motivation of DPO is to avoid training a RM. You can't take the negative randomly? (needs some justification)} \fk{[If we do not use a RM, then we need to use the above approach to collect coarse signals for all collected full response, this will be time-consuming. And the heuristic approach will introduce too much noise, because the completion quality varies with their fundamental capabilities. Training a reward model can help us introduce a confidence margin to reduce noise.]}
Finally, we optimize the LLMs to learn a better policy for generating reliable rationales through Direct Preference Optimization \cite{dpo}, where the contrastive trajectory pairs are annotated by the PRM.
A general comparison between our method and search-based approaches is shown in Figure~\ref{fig:micro-frame}.
% To this end, in this paper, we propose to collect the trajectories of LLMs during reasoning, and use direct preference modeling (DPO) to improve the accuracy of taking actions and deriving new states. Besides, to tackle the problem of weak feedback on intermediate steps, we propose a sampling based method to estimate the expected value when reaching specific states and taking actions.
% We need to clarify the motivation to build reasoning graph here.
% Specifically, we first prompted the LLMs following the style of ReAct~\citep{react} to produce format and clear reasoning process with explicit actions and states~\footnote{We simply treat \textit{Thought} as action while \textit{Observation} as state. We simply overlook \textit{Action} because usally it does not contain too much information}. The temperature is adjusted and multiple responses are sampled from the models. 
% As a starting point, we simply assigned the responses reaching the correct answer with rewards \textbf{1}.


\input{images/micro_framework}

% Summarized our experimental results.
In a nutshell, our contribution can be summarized as follows:
\begin{itemize}
    \item We formulate a novel offline training framework by collecting trajectories and direct preference optimization based on outcome supervision.
    \item We propose an approach to synthesis coarse-grained process rewards without the help of teacher models or humman annotation.
    \item We have evaluated our methods on two challenging logical reasoning benchmarks. The results demonstrate significant improvements compared with strong baseline models, which has verified the effectiveness of our proposed method. We also evaluate the quality of generated rationales by \gptf, which shows particular improvement on reasonableness and conciseness compared to our counterparts.
\end{itemize}




==> latex/limitation.tex <==
\section*{Limitations}
The simulation based approach still requires large amount of resources, which has restricted some analysis for our approach, including experiments on competition level code generation that requires long context generation, and those taken on larger policy models.


==> latex/preliminary.tex <==
\section{Preliminary: Reasoning as Planning for LLMs}

Following~\citep{tree-of-thought,rap}, we define the natural language reasoning process as a Markov Decision Process (MDP) with an action-state trajectory: $\tau=\langle\,s_0, a_0,\cdots,s_t,a_t,\cdots,s_T,a_T\,\rangle$, where $a_t$ is the action  taken at timestep $t$ and $s_{t+1}$ is the state that the agent observes after that. 
% Typically, the reasoning process requires several models: (1) a model to take action based on current state $\pi_a\sim p(a|s_t)$; (2) a model managing the state transition $\pi_t\sim p(s|a_t,s_t)$; and (3) a reward model to given feedback to each reasoning step $r_t=r(a_t,s_t)$.
In the context of LLMs, we simplify the setting by considering that both the action and state are sampled from the policy model $\pi_\theta$ (an LLM), such that:
\begin{equation}
    \begin{cases}
        &a_t\sim \pi_\theta(a|c_t), \\
        &s_{t+1}\sim \pi_\theta(s|a_t,c_t), \\
    \end{cases}
\end{equation}
where $\theta$ is the parameter of the policy model, $c_t=(s_0,a_0,\cdots,s_t)$ is the history trace. Besides, a reward model $r_t=r(a_t,s_t)\in\mathbb{R}$ is employed to assess the feasibility and desirability of each state-action pair.
% And it also includes a reward model $r_t=r(a_t,s_t)$ to provide assessment to each state-action pair.

In order to infer a correct answer to a query, the objective of reasoning can be modeled as a search to find the trajectory with the highest expected utility (accumulated rewards).
% where each action-state pair can be interpreted as reasoning step. 
% This process can be time consuming considering the reward is acquired only if the state is really approached, and the exploration space is really huge.
% \citet{rap} propose the framework of reasoning-as-planning to
\citet{rap} propose to accelerate this process by utilizing Monte Carlo Tree Search~\citep{bandit-mct-planning,mcts} to estimate the expected future reward of each node. MCTS maintains a state-action value function $Q(s,a)$ to find high-reward reasoning trajectories efficiently with proper balance between exploration and exploitation.

Nevertheless, incorporating MCTS into the decoding process of LLMs still lead to high latency and cost, 
because the estimation and update of $Q(s,a)$ relies on real-time simulations, where the subsequent states reached by performing an action $a_t$ to a state $s_t$ should be visited recursively to collect the local rewards $r_t$, and the computation of local rewards is often provided by the LLMs themselves.
% which is mainly due to two reasons: (1) most approaches employ LLMs to give self-feedback to each state-action, which introduces extra consumption due to frequent verification. And (2), the estimation of $Q(s,a)$ in MCTS relies on real-time simulation, and each state could be visited multiple times to achieve more accurate approximation. 

% Intuitively, the agents can be directly optimized by $Q(s,a)$ and the final outcome via reinforcement learning without ground-truth trajectories, where $Q(s,a)$ is also referred as Process Reward Model (PRM) \citep{verify-step-by-step}, and the final outcome can be used to define the Outcome Reward Model (ORM). The main challenge is how to design the process reward function without manual labels, and we will introduce it in the following sections.

Naturally, the online planning process can be imitated by offline learning~\citep{alphago}, where  the value  function $Q(s,a)$ can be approximated by learning through offline simulated trajectories. Further more, to omit the online search process, the policy network can be directly optimized towards high $Q(s,a)$ through reinforcement learning (RL). {Thus, the key challenge lies in how to approximate $Q(s,a)$.}
% \sj{Compared with applications in games, e.g., Go and Sudoku, this step is also necessary because the action space in natural language reasoning is dynamic and unconstrained. And the state transition also requires the reasoning ability of policy model. 
% } \sj{$\rightarrow$ The above colored sentences need to be revised. The logic and clarify is not good}
% Finally, this approach aligns with process supervision~\citep{lets-verify}, where the local rewards are estimation of truthful judgement for each reasoning step from human experts. 
\citet{lets-verify} choose to employ human annotations for reward model training. Though effective, the cost and annotation difficulty hinder its  usage to more complex and diverse domains.
In this paper, we attempt to explore how to utilize offline simulation and trajectory collection to avoid the expensive annotation of process supervision, and improve the reasoning ability of LLMs via {supervised preference learning for planning}.
% learned planning \sj{through supervised preference learning}.



==> tables/logical-reasoning.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental results on logical reasoning benchmarks. The subscript refer to the dataset used for fine-tuning. \textit{Lq.} is the short of LogiQA-v2 and \textit{Rc.} is the short for ReClor. \textit{SC.} refers to self-consistency, where the number of sampled solutions is set 5 with temperature as 1.0.}
    \vskip 0.05in
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{3.5mm}{
    \scalebox{0.85}{
    \begin{tabular}{l|ccccc}
    \toprule
                                &  \multicolumn{2}{c}{LogiQA-v2}  & \multicolumn{2}{c}{ReClor} \\
                                & Dev.  & Test & Dev.  & Test \\ \hline
    \chat
    % \footnote{The GPT-3.5 model id is \textbf{gpt-3.5-turbo-1106}.}
                                % & 54.5  & 53.1 & 58.8  & 57.7 \\
                                & 46.0  & 45.4 & 53.2  & 53.7 \\
    \gptf-Turbo
    % \footnote{The GPT-4 model is \textbf{gpt-4-1106-preview}. Due to limited budget, we only evaluate the development set of ReClor and the first 500 questions in the development set of LogiQA-v2.}
                                & 68.0  & ---  & 82.8  & --- \\ \hline
    Llama2-70B-chat             & 45.9  & 43.8  & 55.8 & 60.4 \\
    Mixtral-8$\times$7B-Instruct
                                & 42.2  & 49.5  & 50.0  & 56.7 \\\hline
    \ft{Llama2-7B-SFT}{Rc.}     & 48.1  & \textbf{44.5  }& 49.0  & 48.8  \\ 
    \ft{Llama2-7B-DPO}{Rc.}     & \textbf{51.6} & 47.5  & \textbf{55.1}  & 51.3  \\ %54.2+55.6+55.4 | 51.7+50.5+51.8=
    \ft{Llama2-7B-pDPO}{Rc.}    & 50.2  & 47.4  & 54.0  & \textbf{53.5} \\ % 54.4+53.6+53.4  | 52.5+52.6+55.4
    \midrule
    \ft{Llama2-7B-SFT}{Lq.}     & 46.1  & 45.5  & 65.8  & 53.4 \\
    \ft{Llama2-7B-DPO}{Lq.}     
                                % & 54.4  & 54.4  & 74.4  & 60.1 \\  % Checkpoint-1200
                                & 55.8  & 53.1  & 74.2  & 60.4  \\
    ~~+ \textit{SC. (tem.=1.0, n=5)}
                                % & 56.7  & 54.8  & 76.7  & 60.5  \\
                                & 57.2  & 54.5  & 77.3  & 60.9  \\ 
    \ft{Llama2-7B-pDPO}{Lq.}    & \textbf{56.4}  & \textbf{55.5} & \textbf{75.9}  & \textbf{61.7} \\  % checkpoint-1200
    ~~+ \textit{SC. (tem.=1.0, n=5)}
                                & 56.9  & \textbf{57.0}  & 76.7  & \textbf{61.9} \\
    \bottomrule
    \end{tabular}
    }}
    \label{tab:logic-reason}
    \vspace{-0.2cm}
\end{table} 
